InvGAN: Invertible GANs

Generation of photo-realistic images, semantic editing and representation learning are a few of many potential applications of high resolution generative models. Recent progress in GANs have established them as an excellent choice for such tasks. However, since they do not provide an inference model, image editing or downstream tasks such as classification can not be done on real images using the GAN latent space. Despite numerous efforts to train an inference model or design an iterative method to invert a pre-trained generator, previous methods are dataset (e.g. human face images) and architecture (e.g. StyleGAN) specific. These methods are nontrivial to extend to novel datasets or architectures. We propose a general framework that is agnostic to architecture and datasets. Our key insight is that, by training the inference and the generative model together, we allow them to adapt to each other and to converge to a better quality model. Our \textbf{InvGAN}, short for Invertible GAN, successfully embeds real images to the latent space of a high quality generative model. This allows us to perform image inpainting, merging, interpolation and online data augmentation. We demonstrate this with extensive qualitative and quantitative experiments.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{For photo editing purposes the background is as important as the foreground. However in a GAN framework the background gets less attention as compared to the foregrounds since the background often has less inter sample regularity as compared to foreground object. Hence, during inversion often the background is not accurately inverted. Furthermore small objects such as earrings often gets lost or modified during the inversion and regeneration process. All in all the proposed method can use some pixel level fidelity boost if it to establish itself as a drop in image editing tool.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{As with any high quality generative mechanism our method can also be potentially abused to create fake content. However since our method simply extends the GAN framework to include an inference module, the fake content created will still inherit the tail tail sign of the underlying generative model used. So we expect that the algorithm proposed can not out weigh disproportionately the underlying generative model.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We are in the process of cleaning up and will make our source code publicly available for research purposes.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We use the official train, validation, Test splits.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{However we do not include standard deviations in the reported numbers as they are insignificantly small and only contributes to clutter.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We use V100 32GB and 16GB GPUS for all experiments. For celebA we use 8 GPUs, for MNIST 1 GPU and FFHQ 8 GPUS. We use also 8-V100 GPUS for patch based BIG-GAN training.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We borrow the GAN architecture and training hyper parameters from existing literature, e.g. StyleGAN, DC-GAN and BIG-GAN. We duely acknowledge this.}
  \item Did you mention the license of the assets?
    \answerYes{In out accompanying code. We have retained the original resource licensing.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We intend to provide pre-trained models as our final release but due to space restrictions we haven't made this available with the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We only use publicly available data sets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We use FFHQ data set. It contains high resolution face images. these are potentially personally identifiable data, however, we do not have offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> rebuttal.tex <==
\section{Rebuttal}

We thank all the reviewers for their insightful comments. One suggestion had been to include more comparisons with SOTA. Therefore we have extended our table 1 as follows. Compared to our submitted version it includes more comparisons from the reference Indomain GAN inversion [47] and reference [a] 'Generative Hierarchical Features from Synthesizing Images' as suggested by reviewer ehPo. Qualitative comparisons will appear in the camera ready version.

\begin{table}[]
      \centering
        \addtolength{\leftskip} {-2cm}
        \addtolength{\rightskip}{-2cm}
        \begin{tabular}{l c c c c c c}
            \toprule
             \textbf{models} & \textbf{RandFID}\newline & \textbf{RandRecFID} & \textbf{TsRecFID} & \textbf{IntTsFID} & \textbf{MAE$\pm 1$} & \textbf{run time}\\
             \midrule
             FFHQ [a] & 49.65/14.59 & 56.71/23.93 & -/13.73 & TBC & 0.129 & 0.045 \\
             FFHQ Enc.[47] & 46.82/14.38 & -/- & 88.48 / - & -/- & 0.460 \\
             FFHQ MSE opt.[47] & 46.82/14.38 & -/- & 58.04 / - & -/- & 0.106 \\
             FFHQ In-D. Inv.[47] & 46.82/14.38 & 52.02/- & 42.64 / - & TBC & 0.115 & 99.76 \\
             
             \midrule
             DCGAN, MNIST & $17.44/6.10 $ & $16.76/4.25 $ & $17.77/4.70$ & $26.04/11.44 $  & $0.070$ & $3.3*10^{-5}$\\
             StyleGAN, CelebA & $26.63/4.81 $ & $24.35/3.51 $ & $24.37/4.14 $ & $32.37/15.60 $ & $0.150$ & $1.0*10^{-3}$\\ 
             StyleGAN, FFHQ & $49.14/12.12 $ & $44.42/8.85 $ & $41.14/7.15$ & $49.52/14.36 $ & $0.255 $ & $2.0*10^{-3}$\\
             \bottomrule
        \end{tabular}
        \caption{Here we report random sample FID (RandFID), FID of reconstructed random samples (RandRecFID), FID of reconstructed test set samples (TsRecFID), FID of the linear middle interpolation of test set images (IntTsFID) and reconstruction per pixel per color channel mean absolute error when images are normalized between $\pm 1$, also from test set. All FID scores are here evaluated against train set using 500 and 50000 samples. They are separated by `/'. For the traditional MSE optimization based and In-Domain GAN inversion, the MSE errors are converted to MAE by taking square root and averaging over the color channels and accounting for the re-normalization of pixel values between $\pm 1$. Runtime is given in seconds per image. We ran them on a V100 32GB GPU and measured wall clock time. TBC: To be computed. Due to techincal reasons these numbers could not be computed at the moment but will be filled in by camera ready version.}
    \label{tab:fids_and_recon_errors}
\end{table}

\subsection{Reviewer ehPo}
First of all we would like to thank the reviewer for the insightful comments and especially for bringing to our attention the paper titled `Generative Hierarchical Features from Synthesizing Images' (referred to as [a]). Since the paper appeared in CVPR 2021, we did not get hold of it at the time this paper was submitted. None the less this paper sets quite a few benchmarks that are extremely useful for future work and our current paper for comparison.

1. \qheading{Missing comparison:} 
In the camera ready version we will include the following comparisons.
\qheading{Image reconstruction:} The reported FID numbers are directly comparable, we will include the results from [a] into Table 1 of our paper (Please see above in the general comment area.).

\qheading{Image Editing:} We show this in Figure 2 and will include the same sample from [a]. We are happy to elaborate if this need is expressed further. However, since this mainly relies on the generator part which is architecturally the same as vanilla StyleGAN2 and especially since our method generates only one $W$ code for every resolution, unlike [a] whose encoder generates 3 different codes, the style mixing experiment although is highly relevant for [a], is less so for our results. We suspect that a successful or an unsuccessful style mixing would not reveal any new insight about our encoder. Therefore we only pay partial attention in Figure 2. However we are happy to elaborate on this in the camera ready.

\qheading{Image Harmonization:} We perform this in Figure 2. We shall include the results of [a] run on the same images.

\qheading{Evaluation on Discriminative Tasks:} We refrain from venturing into evaluation of learned features on classification tasks since the generative task is purely focused on the data distribution $P(x)$ and can in no way influence learning $P(y|x)$ as proven in `On Causal and Anticausal Learning', Schölkopf et.\ al.\ furthermore a linear probe on generative features is too simplistic a model to reveal feature quality. Perhaps full fine tuning for the discriminative task at hand is a better evaluator but they depend upon the training mechanism, underlying encoder architecture etc. In this light a fair comparison between methods are hard. However, if still desired we can extend classification results from the features extracted from our encoder as in [a].

\qheading{Landmark detection:} This experiment seeks if the inverted code retains detailed special information. This experiment did not cross our mind and we would be happy to include in the camera ready version.

2. \qheading{Strong MAE result for FFHQ In-D:} Mean absolute error or MAE is not a precise measure of quality since they are not shift invariant. This measure is specially unreliable when error falls below a certain threshold. Since the competitive methods already achieve $\sim 5-10\,\%$ error rate instead of comparing directly with their precise values reconstruction FIDs should be relied upon. This metric simply judges if the reconstruction is in the right ballpark.

3. \qheading{Input Image Resolution:} Our main focus is to find an universal GAN inversion procedure, hence we evaluate our method on a variety of models and datasets. Training a high quality StyleGAN on $1024 \times 1024$ resolution is extremely resource heavy and requires mixed precision computation that exhibits instability related to saturating and quantized gradients. Furthermore this is an orthogonal direction of research. Therefore like [a] we choose to not approach $1024 \times 1024$ resolution, although the extension is trivial.

Finally we would like to highlight 2 main differences between [a] and our work. 1) Our work is generator agnostic and does not rely on StyleGAN's hierarchical architecture. 2) Our method does not operate on a pre-trained generator.


\subsection{Reviewer YLEP}
We  thank the reviewer for the positive and constructive feedback. The ethical concerns and potential societal impacts are particularly relevant to us and we appreciate the assessment. 

\qheading{Additional analysis on prediction discrepancy for CelebA classification:} If understood correctly you suggest analyzing the difference in the classifier output rather than the classifier decision. Although this does sound intuitively reasonable, deep classifiers in computer vision tend to be uncalibrated unless explicitly taken care of. The longer the training the more \textit{naively certain} the models get, which renders a comparison of classifier responses as potentially misleading.
    
\qheading{Visualization of generative capabilities:}
We did not explicitly add random samples from the InvGAN models but decided to report the FID scores only, as they are an approximate measure for photo-realistic image quality. It is a general shortcoming of visual presentation that it is unclear to which extent the samples are hand-picked or re-sampled. However we are happy to extend the supplementary materials with an extensive grid of randomly generated images.
    
\qheading{Investigating quality of feature representations:}
As an additional analysis of the embedding quality, we will prepare an evaluation of the shatterability of the latent space. We embed $5000$ CelebA images in the InvGAN latent space and train linear support vector classifiers to predict each CelebA attribute. This experiment will appear in the supplementary material and show that the latent space indeed inherits semantic structure of the data.

\qheading{Ablations on more diverse datasets:}
Extensive ablation studies on high diversity datasets require substantial computational effort. In order to keep the footprint of this work comparatively low, we decided to instead conduct the ablations on the task that is fastest to train on. We agree that more extensive studies on either of the suggested datasets could be a relevant contribution.
    
\qheading{Systematic analysis of model impact:}
We agree that a side-by-side comparison of different backbone GAN architectures, combined with the InvGAN inversion module, would be valuable. However we decided to run the individual experiments using different backbones without hand-picking the dataset-architecture combinations. We expect small differences between, for example, BiGAN and StyleGAN2 caused by the differently constrained latent spaces.
    
\qheading{GAN mode collapse and encoder bias towards majority classes:} We are aware of the GAN mode collapse problem for vastly underrepresented groups. Without having a thorough analysis prepared, we visually confirmed that the GAN inversion does not significantly steer under-represented groups towards over-represented groups (tested on the commonly used protected attribute skin-tone). In fact, the success of model based GAN inversion can alleviate parts of the biased data generation when using GAN methods for augmentation purposes. By using a small fraction of labelled training data it is possible to define a volume in the embedding space that corresponds to a certain protected group. Generating new samples from this area allows for compensating existing biases in purely randomly generated images. This is tangentially related to work from us that is concurrently under submission.



\subsection{Reviewer UA7A}
We thank the reviewer for such an thorough, detailed and well thought of review. This surely shall improve our paper quality. Below we clarify the changes we shall make to incorporate the suggestions made.

1 \qheading{Tiled prediction strategy}: We consider the tiling prediction strategy as one of the application allowed by a fast model based approach. The main take away here is that now we can reach for 2K or even 4K images if we trained StyleGAN at $1024 \times 1024$ resolution. We have not demonstrated this in the paper as StyleGAN training at $1024 \times 1024$ resolution poses significant technical challenges, such as mixed precision training, gradient quantization and saturation instabilities, large video ram consumption and in-availability of larger than $1024 \times 1024$ public data sets. However we would like to showcase that when these orthogonal problems are solved, our method naturally extends to those settings. We shall make this point clearer in the camera ready version.

\qheading{Comparison with SOTA}: We shall include FID comparison and MAE comparison from Adversarial Latent Autoencoders in Table 1. Also we shall include qualitative comparison for style mixing and image harmonization in Figure 2.

\qheading{Quantitative ablation studies}: Pixel wise MSE or MAE are not well correlated to reconstruction quality. Therefore we have tried to avoid such comparison as much as possible. Since it generates false conclusion. One can attempt at identifying how many reconstruction changed class label using a classifier. However that relies on 100\% accuracy of the classifier. We haven't managed to come up with a creative quantitative metric that can measure reconstruction accuracy/quality. We are happy to include any such metric should they come up during this discussion in the camera ready version.

\qheading{Deblurring test setting not clear:} The process is as follows
1. Encode the blurry/low resolution image that we wish to sharpen
2. Further blur the blurry image and encode it
3. Find the direction of blurring
4. Flip the direction of blurring to get direction of sharpening
5. Make a few steps in the sharpening direction

We shall clarify these steps in the camera ready better. We described it with the lines 270 - 277, we shall rephrase it in a more understandable way.

\qheading{Comparison with Vanilla GAN:} We expected on the reader's side that the FIDs would directly be compared with the StyleGAN's official implementation. However we do agree random sample FID from vanilla GAN training from our framework should be included in table 1 for easier and fairer comparison. We shall include in the camera ready.

\subsubsection{Questions}
\qheading{500 image FID:} The images are not exactly the same. We shall include a standard deviation error bar for 500 image FID computation. However FID evaluation suffers from bias error for small number of images. This might not be captured in the error-bar as it will focus on variance. Therefore we would like the reader to base conclusions more on 50K FIDs.

\qheading{Better RandRecFID than Rand FID:} In our experience the FID metric favours precision more than diversity. A reconstruction of radom samples make them ever so slightly be reconstructed more like an average digit. This in our opinion pushes up the FID score marginally.

\qheading{Error interval in Table2:} The results are on held out validation set. The error bars are over different raining runs. We shall include this clarification int the camera ready.



\subsection{Reviewer NKsx:} We thank the reviewer for bringing up the novelty issue and lack of comparison to SOTA. 

\qheading{Lack of novelty:} We will contrast InvGAN against BiGAN and ALI as follows in the camera ready version. In ALI and BiGAN, a discriminator network estimates the divergance between two estimates of the joint distribution of data and its latent distribution $P(x,z)$. One of them is latent code inferred from data together with true data point i.e. $P(x, E(x))$ and the other is generated data together with a latent code sampled from its prior distribution i.e. $P(G(z), z\sim P(z))$. Here G is the generator and E is the encoder. This forces the discriminator to operate in the joint space of images and its latent representation. Now, the joint space is topologically different than either the latent space or the data space. This makes discrimination in the joint space much harder compared to the same task in either of the spaces. Furthermore as deep networks tends to capture more global features as compared to local details the reconstruction from BiGAN and ALI do not correspond to each other in pixel wise sense. The only keep very high level semantic correspondences. InvGAN on the other hand wants to force pixel-wise matching between reconstructed image and given image. Therefore the goal is fundamentally different. Furthermore the biggest difference in the method has not so much to do with weight sharing but rather lies in the fact that InvGAN successfully avoids operations in the joint data-latent space (x, z) space. Thereby being able to operate with only one type of data.

\qheading{Missing SOTA comparison:} Thank you very much for pointing this out. This point has been raised universally. We believe that this steams from a flawed assumption on our side: FID numbers are comparable across different papers and therefore we did not mention them again explicitly. However we do see that this generates confusion and difficulty, therefore we shall include several other methods (see rebuttal comments to reviewer UA7A and ehPo and the general comment section up above).

We do not think InvGAN can be fairly compared to ``Encoding in style: a stylegan encoder for image-to-image translation". This is because of the following differences. 1. Encoding in Style uses identity loss. It is unclear how to extend this to non face category. 2. In its full version `Encoding in style' inverts real images to $W+$ space rather than $W$ space. It makes a significant difference since $W+$ space is much larger than $W$. For example, even non-face images can be inverted to $W+$ space of a StyleGAN trained on FFHQ. This will force us to compare with an ablated version 3. `Encoding in style' is a StyleGAN specific paper and it is unclear how this can be extended to other backbone architectures. However we are listening to the comments and if the need is still felt we are happy to include a comparison.
